The variance-penalized stochastic shortest path problem

The stochastic shortest path problem (SSPP) asks to resolve the non-deterministic choices in a Markov decision process (MDP) such that the expected accumulated weight before reaching a target state is maximized. This paper addresses the optimization of the variance-penalized expectation (VPE) of the accumulated weight, which is a variant of the SSPP in which a multiple of the variance of accumulated weights is incurred as a penalty. It is shown that the optimal VPE in MDPs with non-negative weights as well as an optimal deterministic finite-memory scheduler can be computed in exponential space. The threshold problem whether the maximal VPE exceeds a given rational is shown to be EXPTIME-hard and to lie in NEXPTIME. Furthermore, a result of interest in its own right obtained on the way is that a variance-minimal scheduler among all expectation-optimal schedulers can be computed in polynomial time.

==> input/old_example.tex <==



\begin{figure}[h]
  \begin{subfigure}[b]{.4\textwidth}
    \resizebox{1\textwidth}{!}{%
      \begin{tikzpicture}[scale=1,auto,node distance=8mm,>=latex]
        \tikzstyle{round}=[thick,draw=black,circle]

        \node[round, draw=black,minimum size=10mm] (sinit) {$\sinit$};
        \node[round,above=25mm of sinit,minimum size=10mm] (input) {$c$};
        \node[round,right=25mm of input,minimum size=10mm] (t) {$t$};
        \node[round,left=25mm of input,minimum size=10mm] (s) {$s$};

        \draw[color=black ,->,very thick] (sinit)  edge  node [ near start, anchor=center] (m5) {} node [pos=0.2,left=3pt] {$1/2$} (s) ;
        \draw[color=black ,->,very thick] (sinit) edge  node [ near start, anchor=center] (m6) {} node [pos=0.2,right=3pt] {$1/2$} (t) ;
        \draw[color=black , very thick] (m5.center) edge [bend left=35] node [pos=0.5,above=5pt] {$\tau \colon +0$} (m6.center);




        \node[round,above=25mm of input,minimum size=10mm] (goal) {$\goal$};

        \draw[color=black ,->,very thick] (s) edge  node [pos=0.5,below] {$\tau: +0$} (input) ;
        \draw[color=black ,->,very thick] (t) edge  node [pos=0.5,below] {$\tau: +1$} (input) ;

        %
        \draw[color=black ,->,very thick] (input) edge [bend left] node [pos=0.5,left] {$\alpha: +1$} (goal) ;
        \draw[color=black ,->,very thick] (input) edge [bend right] node [pos=0.5,right] {$\beta: +0$} (goal) ;

        %        
        %    
        % \draw[color=black ,->,very thick] (s)  edge  node [ near start, anchor=center] (m5) {} node [pos=0.3,left] {} (t1) ;
        %    \draw[color=black ,->,very thick] (s) edge [bend left=50] node [very near start, anchor=center] (m6) {} node [pos=0.13,right=3pt] {} (input) ;
        %    \draw[color=black , very thick] (m5.center) edge [bend left=35] node [pos=0.75,above=15pt] {$\wgt \colon +1$} (m6.center);
        %    
        %    
        %    \draw[color=black ,->,very thick] (t) edge [bend right=50] node [very near start, anchor=center] (n5) {} node [pos=0.2,left=2pt] {} (input) ;
        %    \draw[color=black ,->,very thick] (t) edge node [ near start, anchor=center] (n6) {} node [pos=0.28,right] {} (t3) ;
        %    \draw[color=black , very thick] (n5.center) edge [bend left=35] node [pos=0.3,above=10pt] {$\wgt \colon +2$} (n6.center);
        %    
        %       
        %     \draw[color=black ,->,very thick] (t1) edge  node [pos=0.4,below=3pt] {$\wgt: +5$} (goal) ;
        %          \draw[color=black ,->,very thick] (t3) edge node [pos=0.4,below=3pt] {$\wgt: +2$} (goal) ;
        %    
        %    

      \end{tikzpicture}
    }
  \end{subfigure}
  %
  \hspace{12pt}
  \begin{subfigure}[b]{.5\textwidth}
    \begin{tikzpicture}[yscale=0.8,xscale=.8]
      \begin{axis}[
          axis lines = middle,
          xlabel={$\mathbb{E}$},
          ylabel={$\mathbb{V}$},
          ymin=-.1, ymax=1.1,
          xmin=0, xmax=1.8,
          xticklabels={0,.5,1,1.5},
          yticklabels={0,.25,.5,.75,1},
          xtick={0,.5,1,1.5},
          ytick={0,.25,.5,.75,1},
        ]
        \addplot [name path=A,domain=.5:1,
          samples=300,
          color=black,thick]
        {1/2-.5*x-(x-.5)*(x-1)};
        \addplot [name path=B,domain=.5:1,
          samples=300,
          color=black,thick]
        {-1/2+1.5*x-(x-.5)*(x-1)};
        \addplot [name path=C,domain=1:1.5,
          samples=300,
          color=black, thick]
        {-1/2+.5*x-(x-1)*(x-1.5)};
        \addplot [name path=D,domain=1:1.5,
          samples=300,
          color=black,thick]
        {5/2-1.5*x-(x-1)*(x-1.5)};

        \addplot [domain=.5:1.5,
          samples=300,
          color=red, very thick]
        {1/4-(x-.5)*(x-1.5)};


        \addplot[black!8] fill between[of=A and B];
        \addplot[black!8] fill between[of=C and D];

        \node[label={0:{$\sched_{\alpha,\alpha}$}},circle,fill,inner sep=2pt] at (axis cs:1.5,.25) {};
        \node[label={180:{$\sched_{\beta,\beta}$}},circle,fill,inner sep=2pt] at (axis cs:.5,.25) {};
        \node[label={[label distance=3pt]176:{$\sched_{\alpha,\beta}$}},circle,fill,inner sep=2pt] at (axis cs:1,0) {};
        \node[label={180:{$\sched_{\beta,\alpha}$}},circle,fill,inner sep=2pt] at (axis cs:1,1) {};
        \node[label={90:{$(\eta,\nu)$}},circle,fill,inner sep=2pt,color=blue] at (axis cs:1.1,.2) {};
        \draw[dashed,thick,color=blue] (axis cs:1.1,.2) -- (axis cs:1.1,0);
        \draw[dashed,thick,color=blue] (axis cs:1.1,.2) -- (axis cs:1.8,.2);
      \end{axis}
    \end{tikzpicture}
  \end{subfigure}
  %
  \caption{The left hand side shows the  MDP $\cM$ for Example \ref{ex:intro}. On the right hand side, all possible combinations of expected accumulated weight and variance that can be achieved by schedulers for $\cM$ are depicted as a gray area. The points corresponding to the four deterministic schedulers are marked. Furthermore, the red line indicates  all combinations  of values that can be achieved by memoryless schedulers.}
  \label{fig:ex_intro}
\end{figure}


\begin{example}\label{ex:intro}
  Consider the MDP $\cM$ depicted in Figure \ref{fig:ex_intro}. We want to analyze the possible trade-offs between the variance and the expected value of the accumulated weight that we can achieve by various schedulers.

  Let us first take a look at deterministic schedulers:
  In state $c$, a choice between actions $\alpha$ and $\beta$ has to be made. As there are two paths leading to state $c$, there are four deterministic schedulers. For $\gamma_0,\gamma_1\in \{\alpha,\beta\}$, let us denote the scheduler that chooses $\gamma_0$ if the accumulated weight in $c$ is $0$ and $\gamma_1$ if the accumulated weight is $1$ by $\sched_{\gamma_{0},\gamma_{1}}$. As under all deterministic schedulers, there are only two paths, we can easily compute expectation and variance under these schedulers. The results are depicted on the right hand side of Figure \ref{fig:ex_intro}.

  If we now start to randomize, by following two different schedulers $\sched$ and $\tsched$ with probability $p$ and $1-p$, respectively, for some $p\in(0,1)$, we will see in Section \ref{sec:two_thresholds} that the expected values and variances under the resulting schedulers lie on a parabolic line segment that is uniquely determined by the expected values and variances of the accumulated weight under $\sched$ and $\tsched$. The area of all feasible combinations of expectation and variance is marked in gray. Note that the black borders of this region are precisely such parabolic line segments resulting from the randomization over two deterministic schedulers.

  The red line segment corresponds to the randomization over the scheduler always choosing $\alpha$ and the scheduler always choosing $\beta$. Hence, the red line segment contains all combinations of expectation and variance that can be achieved by memoryless schedulers.

  A typical multi-objective verification question now asks whether, given two rationals $\eta$ and $\nu$, there is a scheduler $\sched$ such that the expected accumulated weight under $\sched$ is at least $\eta$ while the variance of the accumulated weight is at most $\nu$ under $\sched$.
  For $\eta=1.1$ and $\nu=0.2$, the region indicated by the dashed blue lines in Figure \ref{fig:ex_intro}
  consists of the combinations of expectation and variance that we are looking for. We see that no point corresponding to a deterministic scheduler or a memoryless scheduler lies in this region. So, memory and randomization are necessary to find a scheduler as desired.
  However, there clearly are schedulers satisfying both threshold constraints: For example, consider the scheduler $\rsched$ that always chooses $\alpha$ when the accumulated weight in $c$ is $0$ and that chooses $\alpha$ with probability $1/4$ if the accumulated weight in $c$ is $1$.
  Under this scheduler $\rsched$, the trap state $\goal$ is reached with weight $1$ with probability $7/8$ and with weight $2$ with probability $1/8$.
  The expected accumulated weight is hence
  \[
    7/8\cdot 1 +  1/8 \cdot 2 = 9/8 \geq \eta
  \]
  while the variance is
  \[
    7/8 \cdot (1-9/8)^2 + 1/8 \cdot (2-9/8)^2 = 7/64 \leq \nu.
  \]
  As $\rsched$ is obtained by randomizing over schedulers $\sched_{\alpha,\beta}$ and $\sched_{\alpha,\alpha}$, the corresponding point $(9/8,7/64)$ lies on the black parabolic line segment in the region right below the point $(\eta,\nu)$.
\end{example}

==> input/two_thresholds.tex <==


\section{Threshold conditions on expectation and variance}\label{sec:two_thresholds}

\textcolor{blue}{
	Is there a scheduler with expected accumulated weight  $\geq \eta$ and variance $\leq \nu$?}

\textcolor{blue}
{Possibly a hardness result?}

\textcolor{blue}
{
	Even undecidability?}

\textcolor{blue}
{
	Approximate Pareto-curve (efficiently) computable?}


\textcolor{blue}{Two related questions:
	\begin{enumerate}
		\item
		      What shape does the Pareto-curve have? Convex/concave?
		\item
		      Given two schedulers $\sched$ and $\tsched$, what are the expected value and the variance of a convex combination
		      ``$p\cdot \sched + (1-p)\cdot \tsched$''?
	\end{enumerate}
	(For expected value, it's clear, but not so for the variance.)
	\[
		\Var(p\cdot X + q\cdot Y)=p^2\Var(X)+2p(1-p)\mathrm{Cov}(X,Y)+q^2\Var(Y)
	\]
}


The optimization of variance-penalized expectation in the previous section provides a tool to compute schedulers that are \emph{Pareto-optimal}.
If a scheduler maximizes the variance-penalized expectation for some parameter $\lambda$, there is no scheduler with the same of a higher expectation while having at most the same variance, and vice versa. Different choices of the parameter $\lambda$, moreover, allow to achieve different tradeoffs between variance and expectation.

In this section, we now investigate the following multi-objective problem: Given an MDP $\cM$ with a designated trap state $\goal$ and rational values $\eta$ and $\nu$, is there a scheduler $\sched$ such that
\[
	\mathbb{E}^{\sched}_{\cM}(\rawdiaplus \goal) \geq \eta \qquad \text{ and } \qquad \Var^{\sched}_{\cM}(\rawdiaplus \goal) \leq \nu ?
\]
In this question, the desired tradeoff between variance and expectation can directly be given in terms of these two thresholds.

\begin{definition}[Feasible points, realizable points]
	Given an MDP $\cM$ with a designated trap state $\goal$, we call a point $(\eta,\nu)\in \mathbb{R}^2$ \emph{feasible} if there is a scheduler $\sched$ with
	\[
		\mathbb{E}^{\sched}_{\cM}(\rawdiaplus \goal) \geq \eta \qquad \text{ and } \qquad \Var^{\sched}_{\cM}(\rawdiaplus \goal) \leq \nu.
	\]
	We call the point $(\eta,\nu)$ realizable if there is a scheduler $\sched$ with
	\[
		\mathbb{E}^{\sched}_{\cM}(\rawdiaplus \goal) = \eta \qquad \text{ and } \qquad \Var^{\sched}_{\cM}(\rawdiaplus \goal) = \nu.
	\]
\end{definition}


In the sequel, we study the region of feasible points. Given two points $(x,y)$ and $(x^\prime,y^\prime)$ in $\mathbb{R}^2$, we define the following domination relation:
\[
	(x,y) \succeq (x^\prime,y^\prime) \qquad \text{ iff } \qquad x\geq x^\prime \text{ and } y\leq y^\prime.
\]
The region of feasible points is now the downwards closure with respect to $\succeq$ of the region of the realizable points.


\tudparagraph{1ex}{Convex combination of schedulers.}
As a first step to understand the structure of the feasible region, we take a look at convex combinations of schedulers. Given two schedulers $\sched$ and $\tsched$ and the corresponding points in the realizable region, the following lemma tells us where the points in the realizable region corresponding to the
schedulers $p\cdot \sched \oplus (1-p)\cdot \tsched$ (see Definition \ref{def:convex_scheduler}) for $p\in [0,1]$ lie.


\textcolor{red}{Lemma moved}

\begin{remark}
Given two schedulers $\sched$ and $\sched^\prime$ under which the expectation and variance are $(\eta,\nu)$ and $(\eta^\prime,\nu^\prime)$, respectively, such that $\eta<\eta^\prime$,
there is a unique convex combination $\tsched$ of the two schedulers with expectation $x$ for all $x\in [\eta,\eta^\prime]$.
Viewing the variance of these convex combinations as a function $V:[\eta,\eta^\prime]\to \mathbb{R}$, we can observe the following using the previous Lemma \ref{lem:parabolic}:
\[
V(x)= \nu+\frac{x-\eta}{\eta^\prime-\eta}\cdot(\nu^\prime-\nu) + \frac{x-\eta}{\eta^\prime-\eta}\cdot \frac{\eta^\prime-x}{\eta^\prime-\eta} \cdot (\eta^\prime-\eta)^2 = \nu+\frac{x-\eta}{\eta^\prime-\eta}\cdot(\nu^\prime-\nu)  + (x-\eta)\cdot (\eta^\prime - x).
\]
The coefficient before $x^2$ in this quadratic polynomial hence is always $-1$. Therefore, all parabolic line segments occurring in the diagram plotting possible combinations of expectations and variances are segments of translations of the same parabola.
\end{remark}





\textcolor{red}{Maybe 'feasible points' (for the points currently called 'realizable') and 'dominated points' is better terminology}

\begin{figure}[ht]
	\centering
	\includegraphics[width=0.83\textwidth]{graphics/Pareto_curve.jpg}
	\caption{Sketch of a region of feasible points.}
	\label{fig1}
\end{figure}

Given two realizable points $(\eta,\nu)$ and $(\eta^\prime,\nu\prime)$, this means that all points on the parabolic path
\begin{align*}
	\gamma: [0,1] & \to \mathbb{R}^2                                                                                                            \\
	p             & \mapsto (p\cdot \eta + (1-p)\cdot \eta^\prime, p\cdot \nu + (1-p)\cdot \nu^\prime + p\cdot (1-p) \cdot (\eta-\eta^\prime)^2
\end{align*}
belong to the set of realizable points as well.
Figure \ref{fig1} depicts a sketch of the form of the region of realizable points based on this observation. For any two realizable points, the parabolic path segment connecting these points (which is uniquely determined by the points accoridng to the observation above) belongs to the region of realizable points.

In FIgure \ref{fig1}, the region of feasible points contains everything on the upper left of the points corresponding to the expectation-maximal point (1) and the variance-minimal scheduler (4).
The Pareto-frontier is determined by two further extreme points (2) and (3). Next two point (2), there is a small region of points that are feasible but not realizable.


\tudparagraph{1ex}{Convex hull of the region of feasible points.}
The convex hull of the region of feasible points is indicated by dashed lines between points (1) and (2) as well as (2) and (4).
Feasible points that lie on the border of this convex hull are optimal for the variance-penalized expectation for some parameter $\lambda$.
In the figure, point (1) is optimal for all parameters approximately $\leq 1/2$. Point (2) is optimal for $1/2\leq \lambda \leq 2$ and point (4) is optimal for $\lambda \geq 2$. These values $1/2$ and $2$ for $\lambda$ correspond to the (approximate) reciprocal  slope of the line segments connecting the points.



\textcolor{red}{
	\tudparagraph{1ex}{Questions regarding point (3).}
	Such a point is locally optimal for the variance-penalized expectation for some $\lambda$. I.e., there is an interval $[a,b]$ with $a<b$ and a $\lambda>0$
	such that the scheduler $\sched$ that achieves the maximal value $\VPE[\lambda]^{\sched}_{\cM}$ among all schedulers with $\mathbb{E}^{\sched}_{\cM}(\rawdiaplus\goal) \in [a,b]$ corresponds to this realizable point.
	\begin{itemize}
		\item
		      Are such points realizable by deterministc finite-memory schedulers?
	\end{itemize}
}

\tudparagraph{1ex}{Conjecture regarding the Pareto curve:}
For each feasible point $(\eta,\nu)$, there are two deterministic (finite-memory (?)) schedulers $\sched$ and $\tsched$ and a $p\in[0,1]$ such that
\[
	\mathbb{E}^{p\cdot\sched\oplus(1-p)\cdot\tsched}_{\cM}(\rawdiaplus\goal) \geq \eta
\]
and
\[
	\Var^{p\cdot\sched\oplus(1-p)\cdot\tsched}_{\cM}(\rawdiaplus\goal) \leq \nu.
\]
\textcolor{red}{This could be a key step towards decidability of the question with two thresholds.}


%
%\textcolor{blue}{Stronger version:}
%
%\begin{theorem}
%Let $\cM$ be an MDP with arbitrary integer weights and designated trap state $\goal$.
%Let $(\eta,\nu)\in \mathbb{R}^2$ be given. If there is a scheduler $\sched$ for $\cM$ with 
%\[
%\mathbb{E}^{\sched}_{\cM}(\rawdiaplus \goal) \geq \eta \qquad \text{ and }\qquad \Var^{\sched}_{\cM}(\rawdiaplus \goal) \leq \nu,
%\]
%then there is a weight-based scheduler $\tsched$ and at most one state-weight pair $(s,w)$ such that $\tsched(s^\prime,w^\prime)$ is a Dirac-distribution for all state-weight pairs $(s^\prime,w^\prime)$ different to $(s,w)$ that also satisfies 
%\[
%\mathbb{E}^{\tsched}_{\cM}(\rawdiaplus \goal) \geq \eta \qquad \text{ and }\qquad \Var^{\tsched}_{\cM}(\rawdiaplus \goal) \leq \nu.
%\]
%\end{theorem}
%
%\begin{corollary}
%For each Pareto-optimal scheduler $\sched$, there is a weight-based scheduler $\tsched$ with the same expectation and variance as $\sched$ that uses randomization at most at one state-weight pair.
%\end{corollary}













\tudparagraph{1ex}{Observations regarding VPE-optimal schedulers.}
Given a constant $\Lambda>0$, and $\lambda\geq\Lambda$, an optimal scheduler for the $\VPE[\lambda]$ can be found among deterministic weight-based schedulers with memory only up to a saturation point $K_{\Lambda}$ which does not depend on $\lambda$ but only on $\Lambda$.
So, there are only finitely many points which are optimal for $\VPE[\lambda]$ for some $\lambda\geq \Lambda$.
Hence, except for close to the maximal expectation, there are only finitely many realizable points on the border of the convex hull.

Close to the realizable points with maximal expectation, the points on the border of the convex hull are optimal for small values $\lambda$. As the saturation point grows when $\lambda$ tends to $0$, there might be infinitely many realizable points on the border of the convex hull.
\textcolor{red}{Here, problems with decidability might arise.}







\subsection{Hardness}
Let us call the following the \emph{threshold problem}:
given MDP~$\cM$, and bounds~$\eta, \nu$, determine whether there exists a scheduler $\sched$ such that
\[
	\mathbb{E}^{\sched}_{\cM}(\rawdiaplus \goal) \geq \eta \qquad \text{ and } \qquad \Var^{\sched}_{\cM}(\rawdiaplus \goal) \leq \nu.
\]

Section~\ref{sec:minimal_variance} established that this problem is in PTIME when~$\eta\geq \mathbb{E}^{\max}_{\cM}[\rawdiaplus\goal]$.
Here, we prove EXPTIME-hardness in the general case, and PSPACE-hardness for acyclic MDPs.

We provide reductions from the problem of determining the existence of a scheduler~$\sched$ satisfying $\mathbb{P}^{\sched}_{\cM}[\rawdiaplus\goal=T]=1$,
which was shown to be EXPTIME-complete for MDPs with nonnegative weights in which all schedulers are proper in~\cite{HaaseKiefer15},
and PSPACE-complete on acyclic MDPs.

\begin{theorem}
	The threshold problem is EXPTIME-hard for MDPs with nonnegative weights, even when $\eta=\nu=0$.
	It is PSPACE-hard if on acylic MDPs with nonnegative weights, even when $\eta=\nu=0$.
\end{theorem}
\begin{proof}
	Consider an MDP~$\cM$ with nonnegative weights in which all schedulers are proper, and a value~$T$.
	Define~$\cM'$ by adding a fresh initial state $\iota$ from which a unique action (with weight~$0$) leads, with probability $1/2$, to
	the initial state of~$\cM$;
	while with probability $1/2$ it leads to a fresh state $\iota'$. From~$\iota'$, a unique action with weight~$T$ leads to $\goal$.

	Then, there exists a scheduler $\sched'$ with $\mathbb{P}^{\sched}_{\cM}[\rawdiaplus\goal=T]=1$
	iff
	there exists $\sched'$ with $\mathbb{V}^{\sched'}_{\cM'}[\rawdiaplus\goal] = 0$.

	In fact, $\mathbb{V}^{\sched'}_{\cM'}[\rawdiaplus\goal] = 0$ means that almost all paths have the same value $\rawdiaplus\goal$;
	but since under all schedulers, the path going through $\iota,\iota',\goal$ has probability $1/2$, we must have
	$\mathbb{P}^{\sched'}_{\cM'}[\rawdiaplus\goal=T]=1$; thus we can define~$\sched$ such that $\mathbb{P}^{\sched}_{\cM}[\rawdiaplus\goal=T]=1$.
	Conversely, if $\mathbb{P}^{\sched}_{\cM}[\rawdiaplus\goal=T]=1$, then any scheduler~$\sched'$ for~$\cM'$
	satisfies $\mathbb{P}^{\sched'}_{\cM'}[\rawdiaplus\goal=T]=1$, which means
	$\mathbb{V}^{\sched'}_{\cM'}[\rawdiaplus\goal]=0$.

	Since~$M$ and~$M'$ only have nonnegative weights, the bound~$\eta$ is trivially satisfied.
	Moreover, $\cM'$ is acylic iff $\cM$ is acyclic.
	Both lower bounds then follow from \cite{HaaseKiefer15}.
\end{proof}

%
%\noindent{\bf Conjecture: }
%Given an MDP $\cM$ with a designated trap state $\goal$, no  end components, and weights in $\mathbb{Z}$, and a rational $\vartheta$, the problem whether
%\[
%\Var^{\min}_{\cM}(\rawdiaplus \goal) < \vartheta
%\]
%is Positivity-hard.
